A Spring Propelled Extreme Environment Robot for Off-World Cave Exploration

Pits on the Moon and Mars are intriguing geological formations that have yet to be explored. These geological formations can provide protection from harsh diurnal temperature variations, ionizing radiation, and meteorite impacts. Some have proposed that these underground formations are well-suited as human outposts. Some theorize that the Martian pits may harbor remnants of past life. Unfortunately, these geo-logical formations have been off-limits to conventional wheeled rovers and lander systems due to their collapsed ceiling or 'skylight' entrances. In this paper, a new low-cost method to explore these pits is presented using the Spring Propelled Extreme Environment Robot (SPEER). The SPEER consists of a launch system that flings disposable spherical microbots through skylights into the pits. The microbots are low-cost and composed of aluminium Al-6061 disposable spheres with an array of adapted COTS sensors and a solid rocket motor for soft landing.By moving most control authority to the launcher, the microbots become very simple, lightweight, and low-cost. We present a preliminary design of the microbots that can be built today using commercial components for under 500 USD. The microbots have a total mass of 1 kg, with more than 750 g available for a science instrument. In this paper, we present the design, dynamics and control, and operation of these microbots. This is followed by initial feasibility studies of the SPEER system by simulating exploration of a known Lunar pit in Mare Tranquillitatis.

==> layout.tex <==
introduction
* mars and moon are harsh and inhospitable
    * radiation
    * temperature
    * meteorites
    * suggest living underground
* natural pits on moon and mars
    * recent discovery
    * cannot view from orbit
        * need to see inside before we can go there

motivation
* rovers cannot go in pits/caves
    * extreme terrain
        * collapsed ceilings
        * big drops
        * slopes/walls
    * rock ceiling blocks signal
        * cannot control or receive data from rover (no teleoperation)
objective
* derisk exploration of caves and pits
    * use disposable robots to take photos and scans of the inside
        * they don't have to come back to be successful (rover cannot get stuck inside)
        * LOS relay thru rover allows teleoperation
    * mass and cost efficient (piggyback on another mission)
* design a rover-mounted cannon to fire disposable sensor balls into cave/pit

related works
* axel
* spherex

design overview (short)
* spring loaded by winch
* spin ball to vector thrust
* release spring, ball launched into cave/pit
* ball flies and maps
* ball soft-lands
* instrument unpack/science begins
    * rover as relay

method
* ball must not break on landing
    * soft land
        * liquid thrusters too heavy
        * solid rocket motor
        * how will we align thrusters?
    * fast reaction wheels would be very heavy
        * spin stabilization along thrust axis instead
        * precession to burn off excess fuel


* spring launcher design
* rover mounting
* spin stabilized along thrust axis

analysis
* force/energy launch analysis
    * winch, spring
* soft-land analysis 
    * spin analysis
        * null rotational errors
        * wheels on cad
    * thrust analysis
        * solid rocket motor
        * "vector" motor with off-axis spin
        
future work
* design a specification
    * allow universities to contribute instrument balls
        * involve public with NASA
        * prepare future NASA planetary roboticists

conclusion
